The Min-Cut Formulation of Ollivier-Ricci Curvature

Computing Ollivier-Ricci curvature normally requires a local distance matrix and a linear program per edge, prompting workarounds based on entropic regularization or combinatorial proxies. We show that exact curvature needs neither. For any one-step measures, the Kantorovich dual has an integral three-level optimum, reducing each edge to one minimum s-t cut on a distance-free network linear in the read adjacency lists. This solves instances requiring quadratically many distance queries in linear time, while a converse reduction shows that no exact algorithm can beat bipartite matching. Our solver is a median 6 times (up to 506 times) faster than distance construction plus $\mathtt{POT}$'s C++ simplex, 441 times faster than $\mathtt{GraphRicciCurvature}$, and 23 times faster than graph min-cost flow. The whole-graph times of $\mathtt{POT}$ are estimated from a degree-stratified sample of edges, with every edge whose local distance matrix would exceed $5\cdot 10^7$ entries counted at zero time, so up to sampling error they are lower bounds. Even given the distances, Sinkhorn iterations at $\mathtt{GraphRicciCurvature}$'s regularization are a median 12 times slower, and combinatorial proxies alter edge rankings, missing the bulk of the most negatively curved ones.

==> generated/solver_numbers.tex <==
% generated by experiments/artifacts.py -- do not edit
\makeatletter
\@namedef{res@ArtifactsFonts}{type1}
\@namedef{res@ArtifactsLayout}{onecolumn}
\@namedef{res@ArtifactsMethod}{orcut}
\@namedef{res@ECalibGraphs}{Epinions and DBLP}
\@namedef{res@ECalibNodeTypes}{3}
\@namedef{res@ECalibPotSpreadMax}{\ensuremath{1.1\times}}
\@namedef{res@ECalibRatioSpreadMax}{\ensuremath{1.3\times}}
\@namedef{res@ECalibSolveRatioMax}{\ensuremath{2.2\times}}
\@namedef{res@ECalibSolveRatioMin}{\ensuremath{1.2\times}}
\@namedef{res@ECalibTimeSpreadMax}{\ensuremath{1.3\times}}
\@namedef{res@EDasGraphflowOverOursMax}{\ensuremath{32\times}}
\@namedef{res@EDasGraphflowOverOursMin}{\ensuremath{2.8\times}}
\@namedef{res@EDasMaxN}{1{,}048{,}576}
\@namedef{res@EDasOursMaxTime}{158\,s}
\@namedef{res@EDasPotMaxN}{65{,}536}
\@namedef{res@EDasPotOverOursMax}{\ensuremath{5.16\times10^{5}\times}}
\@namedef{res@EDasPotOverOursMin}{\ensuremath{8{,}156\times}}
\@namedef{res@EDasSlopeMax}{1.6}
\@namedef{res@EDasSlopeMin}{1}
\@namedef{res@EFiveGraphs}{15}
\@namedef{res@EFiveGrcMixHubMaxErr}{0.40}
\@namedef{res@EFiveGrcMixMaxErr}{0.40}
\@namedef{res@EFiveGrcMixSlowdownMax}{\ensuremath{2{,}216\times}}
\@namedef{res@EFiveGrcMixSlowdownMedian}{\ensuremath{441\times}}
\@namedef{res@EFiveGrcOtdFullHubMaxErr}{0.037}
\@namedef{res@EFiveGrcOtdFullMaxErr}{0.037}
\@namedef{res@EFiveGrcOtdFullSlowdownMax}{\ensuremath{3{,}071\times}}
\@namedef{res@EFiveGrcOtdFullSlowdownMedian}{\ensuremath{982\times}}
\@namedef{res@EFiveGrcOtdHubMaxErr}{0.34}
\@namedef{res@EFiveGrcOtdMaxErr}{0.34}
\@namedef{res@EFiveGrcOtdSlowdownMax}{\ensuremath{2{,}380\times}}
\@namedef{res@EFiveGrcOtdSlowdownMedian}{\ensuremath{433\times}}
\@namedef{res@EFiveGrcSinkhornHubMaxErr}{0.40}
\@namedef{res@EFiveGrcSinkhornMaxErr}{0.40}
\@namedef{res@EFiveGrcSinkhornSlowdownMax}{\ensuremath{2{,}214\times}}
\@namedef{res@EFiveGrcSinkhornSlowdownMedian}{\ensuremath{708\times}}
\@namedef{res@EFiveJLBoundsHold}{all}
\@namedef{res@EFiveRecallAFThree}{4\%}
\@namedef{res@EFiveRecallBF}{15\%}
\@namedef{res@EFiveRecallGrcAtd}{45\%}
\@namedef{res@EFiveRecallGrcMix}{100\%}
\@namedef{res@EFiveRecallGrcOtd}{100\%}
\@namedef{res@EFiveRecallGrcOtdFull}{100\%}
\@namedef{res@EFiveRecallGrcSinkhorn}{99\%}
\@namedef{res@EFiveRecallJL}{12\%}
\@namedef{res@EFiveSinkhornSmallReg}{0.01}
\@namedef{res@EFiveSinkhornSmallSlowdownMedian}{\ensuremath{5{,}565\times}}
\@namedef{res@EFiveSinkhornTenthMaeMedian}{\ensuremath{6.4\times10^{-3}}}
\@namedef{res@EFiveSinkhornTenthSlowdownMedian}{\ensuremath{12\times}}
\@namedef{res@EFourCutOverFullMax}{\ensuremath{3.1\times}}
\@namedef{res@EFourCutOverFullMedian}{\ensuremath{1.7\times}}
\@namedef{res@EFourGraphflowOverFullMax}{\ensuremath{39\times}}
\@namedef{res@EFourGraphflowOverFullMedian}{\ensuremath{23\times}}
\@namedef{res@EFourGraphflowOverFullMin}{\ensuremath{10\times}}
\@namedef{res@EFourGraphs}{10}
\@namedef{res@EFourMismatches}{0}
\@namedef{res@EFourNoWarmOverFullMax}{\ensuremath{1.9\times}}
\@namedef{res@EFourNoWarmOverFullMedian}{\ensuremath{1.2\times}}
\@namedef{res@EFourNoWarmOverFullMin}{\ensuremath{0.98\times}}
\@namedef{res@EFourNoWitnessOverFullMax}{\ensuremath{1\times}}
\@namedef{res@EFourNoWitnessOverFullMedian}{\ensuremath{0.99\times}}
\@namedef{res@EFourNoWitnessOverFullMin}{\ensuremath{0.96\times}}
\@namedef{res@EFourPotGraphs}{8}
\@namedef{res@EFourPotOverFullMax}{\ensuremath{127\times}}
\@namedef{res@EFourPotOverFullMedian}{\ensuremath{8.1\times}}
\@namedef{res@EFourPotOverFullMin}{\ensuremath{3.8\times}}
\@namedef{res@EFourTwinsMax}{\ensuremath{2.1\times}}
\@namedef{res@EFourWitnessAloneOverFullMax}{\ensuremath{4.2\times}}
\@namedef{res@EFourWitnessAloneOverFullMedian}{\ensuremath{3\times}}
\@namedef{res@EFourWitnessAloneOverFullMin}{\ensuremath{1.1\times}}
\@namedef{res@EOneCertChecked}{56{,}880}
\@namedef{res@EOneCertFailed}{0}
\@namedef{res@EOneEdgeMeasurePairs}{2{,}483{,}155}
\@namedef{res@EOneGraphs}{19}
\@namedef{res@EOneMeasures}{5}
\@namedef{res@EOneOracleMismatches}{0}
\@namedef{res@EOneOrtoolsChecked}{390{,}548}
\@namedef{res@EOneOrtoolsMismatches}{0}
\@namedef{res@EOnePotMaxDiff}{\ensuremath{3.6\times10^{-14}}}
\@namedef{res@EOneVerifyChecked}{9{,}390}
\@namedef{res@EProvFiveSinkhornGraphs}{15}
\@namedef{res@EProvFiveSinkhornMixed}{2}
\@namedef{res@EProvFiveWholeGraphs}{15}
\@namedef{res@EProvFiveWholeMixed}{4}
\@namedef{res@EProvFourGraphs}{10}
\@namedef{res@EProvFourMixed}{0}
\@namedef{res@EProvOpen}{12}
\@namedef{res@EProvRows}{1{,}150}
\@namedef{res@EProvSixMeasuresGraphs}{10}
\@namedef{res@EProvSixMeasuresMixed}{0}
\@namedef{res@EProvSixRadiusGraphs}{8}
\@namedef{res@EProvSixRadiusMixed}{0}
\@namedef{res@ESixBallTwoPotMedian}{\ensuremath{11\times}}
\@namedef{res@ESixCertifiedMin}{100\%}
\@namedef{res@ESixNonLazyLLYRelMax}{\ensuremath{1.3\times}}
\@namedef{res@ESixRelMax}{\ensuremath{5.6\times}}
\@namedef{res@ESixRelMedian}{\ensuremath{0.99\times}}
\@namedef{res@EThreeGraphs}{20}
\@namedef{res@EThreeLargestEdges}{\ensuremath{1.17\times10^{8}}}
\@namedef{res@EThreeLargestName}{Orkut}
\@namedef{res@EThreeLargestTime}{49.6\,h}
\@namedef{res@EThreeOtherMeasuresGraphs}{19}
\@namedef{res@EThreeOtherMeasuresRelMax}{\ensuremath{1.1\times}}
\@namedef{res@EThreePotSolveSpeedupMax}{\ensuremath{13\times}}
\@namedef{res@EThreePotSolveSpeedupMedian}{\ensuremath{2\times}}
\@namedef{res@EThreePotSpeedupMax}{\ensuremath{506\times}}
\@namedef{res@EThreePotSpeedupMedian}{\ensuremath{6\times}}
\@namedef{res@EThreePotSpeedupMin}{\ensuremath{3.2\times}}
\@namedef{res@EThreeScalingDBLP}{\ensuremath{22\times}}
\@namedef{res@EThreeScalingGitHub}{\ensuremath{18\times}}
\@namedef{res@EThreeScalingLiveJournal}{\ensuremath{12\times}}
\@namedef{res@EThreeScalingMax}{\ensuremath{22\times}}
\@namedef{res@EThreeScalingMin}{\ensuremath{12\times}}
\@namedef{res@EThreeScalingThreads}{32}
\@namedef{res@EThreeScalingYouTube}{\ensuremath{16\times}}
\@namedef{res@EThreeShareFastMedian}{10.4\%}
\@namedef{res@EThreeShareWitnessMax}{3.7\%}
\@namedef{res@EThreeShareWitnessMedian}{0\%}
\@namedef{res@EThreeThreads}{32}
\@namedef{res@EThreeTwinMax}{33{,}375}
\@namedef{res@ETwoDistBytesMax}{2{,}048\,MB}
\@namedef{res@ETwoHubGraphflowMax}{\ensuremath{53\times}}
\@namedef{res@ETwoHubGraphflowMin}{\ensuremath{17\times}}
\@namedef{res@ETwoHubLeafPot}{\ensuremath{223\times}}
\@namedef{res@ETwoHubMaxS}{65{,}536}
\@namedef{res@ETwoHubPotMax}{\ensuremath{1{,}609\times}}
\@namedef{res@ETwoHybridArcsPerInputMax}{3}
\@namedef{res@ETwoNoWitnessArcSlopeMax}{1.9}
\@namedef{res@ETwoNoWitnessArcsPerInputMax}{554}
\@namedef{res@ETwoRealGraphflowMax}{\ensuremath{39\times}}
\@namedef{res@ETwoRealGraphflowMedian}{\ensuremath{19\times}}
\@namedef{res@ETwoRealGraphflowMin}{\ensuremath{12\times}}
\@namedef{res@ETwoRealGraphs}{18}
\@namedef{res@ETwoRealPotBuildMedian}{\ensuremath{7\times}}
\@namedef{res@ETwoRealPotMedian}{\ensuremath{2.4\times}}
\@namedef{res@ETwoSymGraphflowMax}{\ensuremath{16\times}}
\@namedef{res@ETwoSymGraphflowMin}{\ensuremath{5.8\times}}
\@namedef{res@ETwoSymGraphflowS}{16{,}384}
\@namedef{res@ETwoSymMaxS}{16{,}384}
\@namedef{res@ETwoSymNoWitnessMax}{\ensuremath{192\times}}
\@namedef{res@ETwoSymNoWitnessMaxRegime}{mixed}
\@namedef{res@ETwoSymNoWitnessMin}{\ensuremath{28\times}}
\@namedef{res@ETwoSymNoWitnessS}{16{,}384}
\@namedef{res@ETwoSymOrtoolsMax}{\ensuremath{2.33\times10^{5}\times}}
\@namedef{res@ETwoSymPotBuildMax}{\ensuremath{15{,}131\times}}
\@namedef{res@ETwoSymPotMax}{\ensuremath{14{,}492\times}}
\@namedef{res@ETwoSymPotMin}{\ensuremath{6{,}603\times}}
\@namedef{res@ETwoSymWitnessAloneMax}{\ensuremath{0.97\times}}
\@namedef{res@ETwoSymWitnessAloneMin}{\ensuremath{0.70\times}}
\@namedef{res@ETwoSymWitnessAloneS}{16{,}384}
\@namedef{res@ETwoWitnessArcSlopeMax}{1}
\@namedef{res@ETwoWitnessArcsPerInputMax}{1.7}
\@namedef{res@EnvCores}{40}
\@namedef{res@EnvCpu}{Intel(R) Xeon(R) Gold 6148 CPU @ 2.40GHz}
\@namedef{res@EnvNetworkx}{3.3}
\@namedef{res@EnvNumba}{0.62.1}
\@namedef{res@EnvNumpy}{2.2.5}
\@namedef{res@EnvOrcut}{1.4.4}
\@namedef{res@EnvOrtools}{9.15.9999}
\@namedef{res@EnvPot}{0.9.7.post1}
\@namedef{res@EnvPython}{3.12.16}
\@namedef{resrows@ablation}{%
two-layer cut, bitsets & 1.3 & 1.7 & 1.0 & 2.6 & 1.5 & 2.3 & 2.2 & 3.1 & 1.5 & 1.7 \\
+ relays $H_1,\dots,H_4$ & 1.3 & 1.6 & 1.1 & 1.8 & 1.3 & 1.6 & 2.1 & 2.9 & 1.4 & 1.5 \\
+ twin merging & 0.99 & 0.99 & 0.97 & 1.3 & 1.2 & 1.2 & 1.8 & 1.3 & 1.4 & 1.0 \\
+ fast path & 0.99 & 0.99 & 0.97 & 1.3 & 1.2 & 1.2 & 1.8 & 1.2 & 1.4 & 0.98 \\
+ warm start & 1.0 & 1.0 & 1.0 & 1.0 & 0.99 & 0.98 & 0.99 & 0.99 & 0.96 & 0.99 \\
+ witness relays (orcut) & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
\midrule
full $-$ all relays & 1.0 & 1.1 & 1.0 & 1.5 & 1.2 & 1.4 & 1.2 & 1.1 & 1.2 & 1.0 \\
full $-$ twins & 1.3 & 1.7 & 1.1 & 1.5 & 1.1 & 1.4 & 1.1 & 2.1 & 1.0 & 1.4 \\
full $-$ fast path & 0.99 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0.98 & 1.1 \\
full $-$ warm start & 1.0 & 0.98 & 0.99 & 1.2 & 1.2 & 1.2 & 1.9 & 1.3 & 1.4 & 0.98 \\
\midrule
witness network alone & 1.1 & 1.8 & 2.4 & 4.2 & 2.8 & 3.7 & 3.3 & 3.4 & 2.9 & 3.2 \\
graph min-cost flow & 30 & 39 & 10 & 30 & 19 & 24 & 23 & 22 & 20 & 23 \\
oracle & 3.3 & 7.2 & 5.2 & 373 & 11 & -- & 59 & 150 & 21 & 8.6 \\
distance matrix + POT & 7.6 & 8.5 & 4.5 & -- & 3.8 & -- & 16 & 127 & 6.4 & 8.9 \\
}
\@namedef{resrows@ablation-head}{%
configuration & \rotatebox{70}{ER} & \rotatebox{70}{BA} & \rotatebox{70}{RGG} & \rotatebox{70}{CL2.1} & \rotatebox{70}{arXiv} & \rotatebox{70}{GitHub} & \rotatebox{70}{Twitch-DE} & \rotatebox{70}{Squirrel} & \rotatebox{70}{Epinions} & \rotatebox{70}{DBLP} \\
}
\@namedef{resrows@approx}{%
GRC default & \ensuremath{1.0\times10^{-14}} & 0.40 & 0.0\% & 1.00 & 100\% \\
GRC OTD & \ensuremath{4.1\times10^{-15}} & 0.34 & 0.0\% & 1.00 & 100\% \\
GRC OTD, all nbrs. & \ensuremath{1.3\times10^{-14}} & 0.037 & 0.0\% & 1.00 & 100\% \\
GRC Sinkhorn & \ensuremath{9.6\times10^{-3}} & 0.40 & 1.3\% & 0.998 & 99\% \\
GRC ATD & \ensuremath{2.8\times10^{-1}} & 0.98 & 17.6\% & 0.755 & 45\% \\
JL mean & \ensuremath{2.9\times10^{-1}} & 0.99 & 5.9\% & 0.734 & 12\% \\
BF & -- & -- & 14.3\% & 0.696 & 15\% \\
AF$_3$ & -- & -- & 14.2\% & 0.388 & 4\% \\
}
\@namedef{resrows@calib}{%
EPYC 7713 & Epinions & 22.9\,s & 89.5\,s & \ensuremath{3.9\times} & \ensuremath{1.4\times} \\
Xeon Gold 6148 & Epinions & 28.8\,s & 90.4\,s & \ensuremath{3.1\times} & \ensuremath{1.3\times} \\
Xeon Gold 6248 & Epinions & 29.1\,s & 85.6\,s & \ensuremath{2.9\times} & \ensuremath{1.2\times} \\
\addlinespace
EPYC 7713 & DBLP & 549\,ms & 4.49\,s & \ensuremath{8.2\times} & \ensuremath{2.1\times} \\
Xeon Gold 6148 & DBLP & 685\,ms & 4.89\,s & \ensuremath{7.1\times} & \ensuremath{2.2\times} \\
Xeon Gold 6248 & DBLP & 688\,ms & 4.50\,s & \ensuremath{6.5\times} & \ensuremath{2.0\times} \\
}
\@namedef{resrows@dasgupta}{%
one pair at distance 1 & 1{,}048{,}576 & 4{,}194{,}308 & 2{,}097{,}160 & 232\,ms & 2.40\,s & 12.2\,ms & 500\,s & 1.0 \\
perfect matching at distance 1 & 1{,}048{,}576 & 6{,}291{,}458 & 7{,}340{,}032 & 1.58\,s & 4.43\,s & 59.1\,ms & 482\,s & 1.2 \\
bounded weighted degrees & 1{,}048{,}576 & 12{,}582{,}914 & 11{,}534{,}336 & 158\,s & 83.9\,min & 770\,ms & 9.71\,h & 1.6 \\
$\sqrt n$ blocks at distance 2 & 1{,}048{,}576 & 6{,}291{,}458 & 4{,}485{,}100 & 1.18\,s & 32.3\,s & 35.9\,ms & 5.14\,h & 1.1 \\
}
\@namedef{resrows@datasets}{%
Deezer & 28{,}281 & 92{,}752 & 172 & 6.56 & \citet{rozemberczki_characteristic_2020} \\
Amazon-Photo & 7{,}487 & 119{,}043 & 1{,}434 & 31.8 & \citet{shchur_pitfalls_2018} \\
Twitch-DE & 9{,}498 & 153{,}138 & 4{,}259 & 32.2 & \citet{rozemberczki_multiscale_2021} \\
Crocodile & 11{,}631 & 170{,}773 & 3{,}546 & 29.4 & \citet{rozemberczki_multiscale_2021} \\
Facebook & 22{,}470 & 170{,}823 & 709 & 15.2 & \citet{rozemberczki_multiscale_2021} \\
Enron & 33{,}696 & 180{,}811 & 1{,}383 & 10.7 & \citet{leskovec_community_2009} \\
AstroPh & 17{,}903 & 196{,}972 & 504 & 22.0 & \citet{leskovec_graph_2007} \\
Squirrel & 5{,}201 & 198{,}353 & 1{,}903 & 76.3 & \citet{rozemberczki_multiscale_2021} \\
Brightkite & 56{,}739 & 212{,}945 & 1{,}134 & 7.51 & \citet{cho_friendship_2011} \\
Amazon-Computers & 13{,}381 & 245{,}778 & 2{,}992 & 36.7 & \citet{shchur_pitfalls_2018} \\
Coauthor-Physics & 34{,}493 & 247{,}962 & 382 & 14.4 & \citet{shchur_pitfalls_2018} \\
GitHub & 37{,}700 & 289{,}003 & 9{,}458 & 15.3 & \citet{rozemberczki_multiscale_2021} \\
Epinions & 75{,}877 & 405{,}739 & 3{,}044 & 10.7 & \citet{richardson_trust_2003} \\
Amazon & 334{,}863 & 925{,}872 & 549 & 5.53 & \citet{yang_defining_2012} \\
DBLP & 317{,}080 & 1{,}049{,}866 & 343 & 6.62 & \citet{yang_defining_2012} \\
roadNet-CA & 1{,}957{,}027 & 2{,}760{,}388 & 12 & 2.82 & \citet{leskovec_community_2009} \\
YouTube & 1{,}134{,}890 & 2{,}987{,}624 & 28{,}754 & 5.27 & \citet{yang_defining_2012} \\
Skitter & 1{,}694{,}616 & 11{,}094{,}209 & 35{,}455 & 13.1 & \citet{leskovec_graphs_2005} \\
LiveJournal & 3{,}997{,}962 & 34{,}681{,}189 & 14{,}815 & 17.3 & \citet{yang_defining_2012} \\
Orkut & 3{,}072{,}441 & 117{,}185{,}083 & 33{,}313 & 76.3 & \citet{yang_defining_2012} \\
}
\@namedef{resrows@exactness}{%
lazy & 19 & 496{,}631 & 95{,}847 / 0 & 0 & \ensuremath{2.8\times10^{-14}} & 12{,}430 / 0 \\
non-lazy & 19 & 496{,}631 & 95{,}847 / 0 & 0 & \ensuremath{3.6\times10^{-14}} & 12{,}430 / 0 \\
Lin--Lu--Yau & 19 & 496{,}631 & 95{,}847 / 0 & 0 & \ensuremath{2.9\times10^{-14}} & 12{,}430 / 0 \\
idleness $1/2$ & 19 & 496{,}631 & 95{,}847 / 0 & -- & \ensuremath{2.2\times10^{-14}} & 12{,}430 / 0 \\
weighted lazy walk & 19 & 496{,}631 & 7{,}160 / 0 & -- & -- & 7{,}160 / 0 \\
}
\@namedef{resrows@large}{%
Deezer & 28{,}281 & 92{,}752 & 172 & 57.4\,ms & 274\,ms & \ensuremath{4.8\times} & 5.8 & 25 \\
Amazon-Photo & 7{,}487 & \ensuremath{1.19\times10^{5}} & 1{,}434 & 1.62\,s & 9.79\,s & \ensuremath{6.1\times} & 429 & 2.5 \\
Twitch-DE & 9{,}498 & \ensuremath{1.53\times10^{5}} & 4{,}259 & 7.67\,s & 59.9\,s & \ensuremath{7.8\times} & 1{,}042 & 9.4 \\
Crocodile & 11{,}631 & \ensuremath{1.71\times10^{5}} & 3{,}546 & 2.30\,s & 303\,s & \ensuremath{131\times} & 220 & 63 \\
Facebook & 22{,}470 & \ensuremath{1.71\times10^{5}} & 709 & 1.29\,s & 4.83\,s & \ensuremath{3.7\times} & 0 & 4.3 \\
Enron & 33{,}696 & \ensuremath{1.81\times10^{5}} & 1{,}383 & 3.68\,s & 17.0\,s & \ensuremath{4.6\times} & 33 & 75 \\
AstroPh & 17{,}903 & \ensuremath{1.97\times10^{5}} & 504 & 1.24\,s & 4.70\,s & \ensuremath{3.8\times} & 0 & 4.5 \\
Squirrel & 5{,}201 & \ensuremath{1.98\times10^{5}} & 1{,}903 & 22.2\,s & 21.6\,min & \ensuremath{59\times} & 855 & 4.8 \\
Brightkite & 56{,}739 & \ensuremath{2.13\times10^{5}} & 1{,}134 & 1.28\,s & 5.80\,s & \ensuremath{4.5\times} & 1.3 & 23 \\
Amazon-Computers & 13{,}381 & \ensuremath{2.46\times10^{5}} & 2{,}992 & 8.10\,s & 71.7\,s & \ensuremath{8.9\times} & 925 & 2.6 \\
Coauthor-Physics & 34{,}493 & \ensuremath{2.48\times10^{5}} & 382 & 514\,ms & 1.66\,s & \ensuremath{3.2\times} & 0 & 3.1 \\
GitHub & 37{,}700 & \ensuremath{2.89\times10^{5}} & 9{,}458 & 14.1\,s & 391\,s & \ensuremath{28\times} & 1{,}396 & 93 \\
Epinions & 75{,}877 & \ensuremath{4.06\times10^{5}} & 3{,}044 & 28.3\,s & 96.2\,s & \ensuremath{3.4\times} & 1{,}105 & 29 \\
Amazon & \ensuremath{3.35\times10^{5}} & \ensuremath{9.26\times10^{5}} & 549 & 332\,ms & 1.99\,s & \ensuremath{6.0\times} & 57 & 52 \\
DBLP & \ensuremath{3.17\times10^{5}} & \ensuremath{1.05\times10^{6}} & 343 & 653\,ms & 4.82\,s & \ensuremath{7.4\times} & 64 & 23 \\
roadNet-CA & \ensuremath{1.96\times10^{6}} & \ensuremath{2.76\times10^{6}} & 12 & 355\,ms & 4.16\,s & \ensuremath{12\times} & 168 & -- \\
YouTube & \ensuremath{1.13\times10^{6}} & \ensuremath{2.99\times10^{6}} & 28{,}754 & 182\,s & 3.10\,h & \ensuremath{61\times} & 6{,}658 & 388 \\
Skitter & \ensuremath{1.69\times10^{6}} & \ensuremath{1.11\times10^{7}} & 35{,}455 & 43.4\,min & 15.3\,d & \ensuremath{506\times} & 14{,}939 & 66 \\
LiveJournal & \ensuremath{4.00\times10^{6}} & \ensuremath{3.47\times10^{7}} & 14{,}815 & 42.9\,min & 3.58\,h & \ensuremath{5.0\times} & 14{,}827 & 9.1 \\
Orkut & \ensuremath{3.07\times10^{6}} & \ensuremath{1.17\times10^{8}} & 33{,}313 & 49.6\,h & 7.91\,d & \ensuremath{3.8\times} & 52{,}547 & 2.8 \\
}
\@namedef{resrows@measures}{%
lazy & 1.0 & 1.0 \\
non-lazy & 1.0 & 1.3 \\
Lin--Lu--Yau & 1.0 & 1.0 \\
idleness $1/4$ & 0.98 & 1.0 \\
idleness $1/2$ & 0.98 & 1.0 \\
idleness $3/4$ & 0.98 & 1.0 \\
weighted lazy walk & 1.0 & 5.6 \\
}
\@namedef{resrows@provenance}{%
E1 & Xeon Gold 6248 (95) \\
E2, controlled edges & four Xeon Gold 6148 (168), Xeon Gold 6248 (75) \\
E2, real graphs & Xeon Gold 6248 (175) \\
E2, lower bounds & four Xeon Gold 6148 (19), Xeon Gold 6248 (9) \\
E3, real networks & Xeon Gold 6248 (57), four Xeon Gold 6148 (1) \\
E3, threads & EPYC 7713 (24) \\
E3, random graphs & EPYC 7713 (56), four Xeon Gold 6148 (20), Xeon Gold 6230 (1), ND (12) \\
E4 & EPYC 7713 (150) \\
E5, whole graphs & EPYC 7713 (63), Xeon Gold 6148 (18) \\
E5, Sinkhorn & Xeon Gold 6148 (90), EPYC 7713 (15) \\
E6, measures & EPYC 7713 (70) \\
E6, balls and walks & Xeon Gold 6148 (32) \\
}
\@namedef{resrows@radius}{%
uniform on $B_{2}$ & 11 & 3.6--21 & \ensuremath{4.5\times10^{-14}} \\
uniform on $B_{3}$ & 6.2 & 0.81--12 & \ensuremath{5.1\times10^{-14}} \\
2-step lazy walk & 13 & 7.9--17 & \ensuremath{3.8\times10^{-10}} \\
3-step lazy walk & 5.5 & 1.6--10 & \ensuremath{6.0\times10^{-10}} \\
}
\@namedef{resrows@synth}{%
BA & avg.~16 & \ensuremath{8.00\times10^{7}} & 1.13 \\
CL2.1 & avg.~16 & \ensuremath{2.02\times10^{7}} & 2.01 \\
CL2.5 & avg.~16 & \ensuremath{7.99\times10^{7}} & 1.57 \\
ER & avg.~16 & \ensuremath{8.00\times10^{7}} & 1.01 \\
RGG & avg.~16 & \ensuremath{7.99\times10^{7}} & 0.93 \\
WS & avg.~16 & \ensuremath{8.00\times10^{7}} & 0.97 \\
BA & $2.1n^{0.4}$ & \ensuremath{4.89\times10^{7}} & 1.85 \\
CL2.1 & $2.1n^{0.4}$ & \ensuremath{6.68\times10^{6}} & 1.86 \\
CL2.5 & $2.1n^{0.4}$ & \ensuremath{9.93\times10^{6}} & 1.96 \\
ER & $2.1n^{0.4}$ & \ensuremath{4.89\times10^{7}} & 1.69 \\
RGG & $2.1n^{0.4}$ & \ensuremath{2.61\times10^{8}} & 1.57 \\
WS & $2.1n^{0.4}$ & \ensuremath{2.64\times10^{8}} & 1.61 \\
}
\@namedef{resrows@threads}{%
DBLP & 32 & \ensuremath{22\times} \\
GitHub & 32 & \ensuremath{18\times} \\
LiveJournal & 32 & \ensuremath{12\times} \\
YouTube & 32 & \ensuremath{16\times} \\
}
\@namedef{resrows@witness}{%
dense & 4{,}096 & 6{,}108{,}502 & 3{,}049{,}130 & 3{,}049{,}130 & 6{,}110{,}548 & 1.0 & 1.0 & 0.99 & 0.89 & 4.0 \\
hubleaf & 16{,}384 & 177{,}610 & 2{,}455{,}787 & 173{,}413 & 173{,}413 & 1.6 & 1.0 & 34 & 0.89 & 7.0 \\
mixed & 16{,}384 & 214{,}822 & 119{,}038{,}847 & 212{,}929 & 212{,}929 & 1.9 & 0.99 & 192 & 0.95 & 9.3 \\
sparse & 16{,}384 & 160{,}262 & 11{,}927{,}732 & 160{,}189 & 160{,}189 & 1.7 & 1.0 & 28 & 0.97 & 5.8 \\
tree & 16{,}384 & 73{,}730 & 32{,}771 & 32{,}771 & 32{,}771 & 0.99 & 0.99 & 81 & 0.70 & 16 \\
}
\makeatother

